MedClaw: Heuristic Agent Harness for Long-Horizon Surgical Video Reasoning

Understanding tens-of-minutes surgical videos requires long-horizon temporal reasoning, answering what happens before, after, or across stages of a procedure by grounding the question in visual evidence spread across time. Existing approaches handle this poorly: a one-shot vision-language model (VLM) compresses the whole procedure to fit its context window and loses the detail a "before" or "after" question depends on, while video agents that train the model where to look are data-hungry and transfer poorly to out-of-domain surgery. We build an agent harness that separates reasoning from perception and improves by evolving context rather than optimizing weights. A text-only orchestrator plans which evidence to gather and issues an auditable sequence of tool calls, while frozen vision-language sub-agents execute each call over the pixels, viewing, cropping, inspecting frames, and retrieving external knowledge. We further propose a gradient-free, reward-gated Heuristic Skill Distillation loop that mines the agent's own low-scoring traces and keeps a candidate skill only when it raises a validation reward, yielding reusable retrieval skills, notably directed re-look. Growing an external skill library rather than tuning weights, the loop adapts from only about 100 labeled examples, far fewer than supervised or reinforcement fine-tuning requires. To evaluate this agent, we introduce MedClawBench, a de-leaked, doctor-grounded benchmark of 1,123 questions over self-built long neurosurgery recordings and a held-out public lecture-video test split. Across both datasets and all four evaluation dimensions, our agent consistently outperforms one-shot VLMs and general video-agent frameworks, with the largest gains on the long, out-of-domain neurosurgery videos. Project page: https://fyycs.github.io/medclaw/.

==> Makefile <==
MAIN := main
LATEXMK := latexmk
LATEXMK_FLAGS := -pdf -interaction=nonstopmode -file-line-error

.PHONY: all pdf force clean distclean

all: pdf

pdf: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(wildcard sec/*.tex) $(wildcard imgs/*) $(MAIN).bib \
             ieeecolor.cls generic.sty
	$(LATEXMK) $(LATEXMK_FLAGS) $(MAIN).tex

force:
	$(LATEXMK) $(LATEXMK_FLAGS) -g $(MAIN).tex

clean:
	$(LATEXMK) -c $(MAIN).tex

distclean:
	$(LATEXMK) -C $(MAIN).tex


==> sec/fig_teaser.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.92\textwidth]{imgs/teaser.pdf}
\caption{MedClaw targets long-horizon surgical video reasoning by pairing a
doctor-grounded, de-leaked benchmark with a frozen-weight agent harness.
Instead of learning a tool-use policy through SFT/RL, a text orchestrator calls
frozen API sub-agents, consults reward-gated skills such as
coarse-to-fine localization and directed re-look, and returns an auditable
evidence trace over the full-length procedure.}
\label{fig:teaser}
\end{figure*}

